IVOIRE Deliverable 1.1: Classification of existing VOs & tools and Formalization of VOs semantics

This report discusses the foundations of the VO approach. Then, it explores multiple directions and argues about structure and applications.

==> requirement_type_technique.tex <==


\begin{table}[t]

\caption{Requirement Types, Criterion Types, and Links to VOs}
\label{tab:links-vo-requirement-criteria}
\resizebox{0.95\textwidth}{!}{
\setlength\tabcolsep{5pt}
\begin{tabular}{l | l}
Requirement/Criterion Type & Validation Obligation \\ \hline
Safety Requirement & LTL, CTL \\ 
Invariant Requirement & + MC, SMC, PO \\
Deadlock-Freedom Requirement & + MC, SMC, PO \\ \hline
Liveness Requirement & LTL, CTL, TR$^1$ \\
(including Livelock-Freedom) & \\ \hline
Use Case Requirement & TR, TRF \\ \hline
Timing Requirement & MC $^2$, LTL $^2$, CTL $^2$, SMC $^2$, PO $^2$, HT $^3$, EOP $^3$ \\ \hline % Simulation VO: SIM?, it is just a base for HT and EOP
Probabilistic Requirement & PSMC, HT, EOP, SISTAT \\ \hline
Enabling Requirement & ED \\ \hline
Read/Write Requirement & RWM \\ \hline
Variable Requirement & MMV \\ \hline
State Space Requirement & SVIS $^4$, STAT $^4$ \\ \hline
Absence of Redundancy Requirement & VAP \\ \hline
Coverage Requirement & OC, MCDC, VCM $^4$, OCT $^4$ \\ \hline
Coverage Criterion & VCM $^5$, OCT $^5$ \\ \hline
State Space Criterion & SVIS $^5$, STAT $^5$ \\ \hline
Projection Criterion & SPRJ $^5$   \\ \hline
Trace Refinement Criterion & TRF $^6$ \\ \bottomrule
\end{tabular}
}
\newline
\footnotesize{$^1$ When an CTL formula requires the existence of a path with a certain property, it could be sufficient to validate the requirement by giving an explicit example representing an execution trace, \newline 
$^2$ depends whether time is part of the model \newline
$^3$ depends on whether time is simulated, probability would be 100\% \newline
$^4$ usually combined with MC \newline
$^5$ usually combined with another VO \newline
$^6$ usually combined with TR}\\
\end{table}



==> validation_tools.tex <==
\begin{table}[ht]
\caption{Overview Validation Techniques}
\label{validation_tools}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{10pt}
\begin{tabular}{l | l |l}
Validation Technique & Parameters & Automatable? \\ \toprule
Composed VO & & \\
Sequence VO & & \\
If-Then VO & & \\ \bottomrule

\end{tabular} 
}
\end{table}

